Evaluating LLMs Effectiveness in Detecting and Correcting Test Smells: An Empirical Study

Test smells indicate poor development practices in test code, reducing maintainability and reliability. While developers often struggle to prevent or refactor these issues, existing tools focus primarily on detection rather than automated refactoring. Large Language Models (LLMs) have shown strong potential in code understanding and transformation, but their ability to both identify and refactor test smells remains underexplored. We evaluated GPT-4-Turbo, LLaMA 3 70B, and Gemini-1.5 Pro on Python and Java test suites, using PyNose and TsDetect for initial smell detection, followed by LLM-driven refactoring. Gemini achieved the highest detection accuracy (74.35\% Python, 80.32\% Java), while LLaMA was lowest. All models could refactor smells, but effectiveness varied, sometimes introducing new smells. Gemini also improved test coverage, unlike GPT-4 and LLaMA, which often reduced it. These results highlight LLMs' potential for automated test smell refactoring, with Gemini as the strongest performer, though challenges remain across languages and smell types.

==> prompts/det_python.tex <==


\begin{tcolorbox}[
    title=Example of Test Smell Detection Prompt for Python,
    breakable,
    colback=white,
    colframe=red!50!black,
    fonttitle=\bfseries,
    boxrule=1pt,
    arc=3mm
]
\ttfamily\small
\textbf{System prompt}\par
\begin{adjustwidth}{2em}{0em}
You are a software quality assurance engineer specializing in Python. Your task is to assure test code quality by detecting test smells.
\end{adjustwidth}\par

\textbf{Definition of test smells:}\par
\begin{adjustwidth}{2em}{0em}
Test smells represent sub-optimal design or implementation solutions applied when developing test cases.
\end{adjustwidth}\par

\textbf{Definition of General Fixture:}\par
\begin{adjustwidth}{2em}{0em}
Occurs when not all fields instantiated within the setUp method of a test class are utilized by all test methods in the same test class.
\end{adjustwidth}\par

\textbf{Follow the steps below to identify this smell within test code}\par
\begin{adjustwidth}{2em}{0em}
\textbf{i)} Analyze the test code provided;\par
\textbf{ii)} According to the General Fixture definition, check if this smell is present in the provided code;\par
\textbf{iii)} Your output should be ‘YES’ if General Fixture is present, and ‘NO’ if it is not present.\par
\end{adjustwidth}\par

\textbf{User Prompt}\par
\begin{adjustwidth}{2em}{0em}
analyze test code below:\newline
\textbf{\{Placeholder\}}
\end{adjustwidth}

\end{tcolorbox}


==> prompts/ref_java.tex <==
\begin{tcolorbox}[
    title=Example of Code Refactoring Prompt for Java,
    breakable,
    colback=white,
    colframe=blue!50!black,
    fonttitle=\bfseries,
    boxrule=1pt,
    arc=3mm,
    enhanced
]
\ttfamily\small
\textbf{System prompt}\par
\begin{adjustwidth}{2em}{0em}
You are an expert Java developer. You will be provided with test code in Java delimited by 4 hashtags and the description of the test smells detected in that code. Your task is to refactor the code in order to eliminate the smells present in the code.
\end{adjustwidth}\par

\textbf{Definition of Conditional Test Logic:}\par
\begin{adjustwidth}{2em}{0em}
Conditional Test Logic occurs when a test method contains one or more control statements (i.e., if, switch, for, foreach and while statements).
\end{adjustwidth}\par

\textbf{User Prompt}\par
\begin{adjustwidth}{2em}{0em}
Refactor the code:\newline
\textbf{\{Placeholder\}}
\end{adjustwidth}

\end{tcolorbox}


==> prompts/ref_python.tex <==
\begin{tcolorbox}[
    title=Example of Code Refactoring Prompt for Python,
    breakable,
    colback=white,
    colframe=red!50!black,
    fonttitle=\bfseries,
    boxrule=1pt,
    arc=3mm,
    enhanced
]
\ttfamily\small
\textbf{System prompt}\par
\begin{adjustwidth}{2em}{0em}
You are a specialist Python developer. You will be provided with test code in Python and a description of a test smell detected in this code. Test smells are patterns in test code that suggest poor design choices. Your task is to refactor the test code to eliminate the test smell present in it.
\end{adjustwidth}\par

\textbf{Definition of Constructor Initialization:}\par
\begin{adjustwidth}{2em}{0em}
The test class utilizes a constructor instead of a setUp method to initialize fields.
\end{adjustwidth}\par

\textbf{Follow the steps below to refactor the Constructor Initialization}\par
\begin{adjustwidth}{2em}{0em}
\textbf{<Step 1>} Analyze the test code provided delimited by 4 hashtags;\par
\textbf{<Step 2>} Understand what this test code is testing, and which test framework is being used;\par
\textbf{<Step 3>} Locate where the Constructor Initialization occurs;\par
\textbf{<Step 4>} Based on the test framework used, refactor this part of the test code to eliminate Constructor Initialization. You can modify the test method as you wish, but keep in mind that you should maintain the test's context;\par
\textbf{<Step 5>} Give me only the test code you refactored.
\end{adjustwidth}\par

\textbf{User Prompt}\par
\begin{adjustwidth}{2em}{0em}
Refactor the code:\newline
\textbf{\{Placeholder\}}
\end{adjustwidth}

\end{tcolorbox}

